Budgeted Matroid Maximization: a Parameterized Viewpoint

We study budgeted variants of well known maximization problems with multiple matroid constraints. Given an $\ell$-matchoid $\cm$ on a ground set $E$, a profit function $p:E \rightarrow \mathbb{R}_{\geq 0}$, a cost function $c:E \rightarrow \mathbb{R}_{\geq 0}$, and a budget $B \in \mathbb{R}_{\geq 0}$, the goal is to find in the $\ell$-matchoid a feasible set $S$ of maximum profit $p(S)$ subject to the budget constraint, i.e., $c(S) \leq B$. The {\em budgeted $\ell$-matchoid} (BM) problem includes as special cases budgeted $\ell$-dimensional matching and budgeted $\ell$-matroid intersection. A strong motivation for studying BM from parameterized viewpoint comes from the APX-hardness of unbudgeted $\ell$-dimensional matching (i.e., $B = \infty$) already for $\ell = 3$. Nevertheless, while there are known FPT algorithms for the unbudgeted variants of the above problems, the {\em budgeted} variants are studied here for the first time through the lens of parameterized complexity. We show that BM parametrized by solution size is $W[1]$-hard, already with a degenerate single matroid constraint. Thus, an exact parameterized algorithm is unlikely to exist, motivating the study of {\em FPT-approximation schemes} (FPAS). Our main result is an FPAS for BM (implying an FPAS for $\ell$-dimensional matching and budgeted $\ell$-matroid intersection), relying on the notion of representative set $-$ a small cardinality subset of elements which preserves the optimum up to a small factor. We also give a lower bound on the minimum possible size of a representative set which can be computed in polynomial time.

==> Algorithm.tex <==
\section{The Algorithm}
\label{sec:alg}

In this section we present an FPAS for the BM problem. 


Our first step is to round the profits of a given instance, and to determine the low profit elements that can be discarded without incurring a significant loss in the profit. Then, we find a small cardinality {\em representative set} from which an almost optimal solution can be selected via enumeration. 

%To this end, we generalize the {\em representative set} notion of \cite{DKS23,doron2023eptas} to the context of parametrized algorithms. 
%Our scheme relies on initially finding a set of profitable elements of small cardinality, from which the most profitable elements are selected for the solution using enumeration. 

 
For the remainder of this section, fix a BC instance $I = (E, \cC, c,p, \beta)$ and an error parameter $0<\eps <\frac{1}{2}$. 
Let $H(I,\eps) = \{e \in E~|~ p(e) > \eps \cdot \OPT(I)\}$ be the set of {\em profitable} elements in $I$, and $E \setminus H(I,\eps)$ the set of {\em non-profitable} elements; when understood from the context, we use $H = H(I,\eps)$. Now, a representative set is a subset of elements which contains the profitable elements of an {\em almost} optimal solution. Formally,
\begin{definition}
	\label{def:REP}
		Let $I = (E, \cm, c,p, B)$ be a \textnormal{BM} instance, $0<\eps<\frac{1}{2}$ and $R \subseteq E$. %be a representatives set of $I$ and $\eps$. 
		Then, $R$ is a {\em representative set} of $I$ and $\eps$ if there is a solution $S$ of $I$ such that the following holds.
	\begin{enumerate}
		\item $S \subseteq R$. 
		\item $p\left(S\right) \geq (1-\eps) \cdot \OPT(I)$.
	\end{enumerate} 
	\end{definition}


The work of \cite{DKS23} laid the foundations for the following notions of {\em replacements} and {\em strict representative sets (SRS)}, for the special case of BC where $\cC$ is a single matroid constraint. Below we generalize the
definitions of replacements and SRS. 

Intuitively, a replacement of a solution $S$ for $I$ of bounded cardinality is another solution for $I$ which preserves the attributes of the profitable elements in $S$ (i.e., $S \cap H$). In particular, the profit of the replacement is close to $p(S \cap H)$, whereas the cost and the number of profitable elements can only be smaller. An SRS is a subset of elements containing a replacement for any solution for $I$ of bounded cardinality. 

The formal definitions of replacement and SRS for general BC instances are given in Definitions~\ref{def:Replacement} and~\ref{def:Representatives}, respectively. Let $q(\eps) = \ceil{\eps^{-\eps^{-1}}}$, and $\cm_{\leq q(\eps)} = \{A \in  \cm ~|~|A| \leq q(\eps)\}$ be all {\em bounded feasible sets} of $\cC$ and $\eps$. Recall that we use $\cm = \cm(\cC)$ for the feasible sets of $\cC$; similar simplification in notation is used also for bounded feasible sets.
 \begin{definition}
	\label{def:Replacement}
	Given a \textnormal{BC} instance $I = (E, \cC, c,p, \beta), 0<\eps<\frac{1}{2}$, $S \in \cm_{\leq q(\eps)}$, and $Z_S \subseteq E$, we say that $Z_S$ is a {\em replacement} of $S$ for $I$ and $\eps$ if the following holds: 
	\begin{enumerate}
		
		\item $(S \setminus H) \cup Z_S \in \cm_{\leq q(\eps)}$.\label{p:I}
		
		\item $c(Z_S) \leq c(S \cap H)$.\label{p:s}
		
		\item $p\left((S \setminus H) \cup Z_S\right) \geq (1-\eps) \cdot p(S)$.\label{p:p}
		
		\item $|Z_S| \leq |S \cap H|$.\label{p:car}
	\end{enumerate}
\end{definition}

 \begin{definition}
\label{def:Representatives}
	Given a \textnormal{BC} instance $I = (E, \cC, c,p, \beta), 0<\eps<\frac{1}{2}$, and $R \subseteq E$, we say that $R$ is a {\em strict representative set (SRS)} of $I$ and $\eps$ if, for any $S \in \cm_{k}$, there is a replacement $Z_S \subseteq R$ of $S$ for $I$ and $\eps$. 
\end{definition}

 
Observe that given any solution $S$ of $I$ such that $|S| \leq q(\eps)$, it holds that $S \cap H$  is a replacement of $S$; also, $E$ is an SRS. In the next result, we demonstrate the power of SRS in solving BC. Specifically, we show that
any SRS $R \subseteq E$ is also a representative set. Hence, using enumeration on subsets of $R$ we can find a subset of elements that can be extended by only non-profitable elements to an {\em almost} optimal solution (see Algorithm~\ref{alg:EPTAS}). 
 
\begin{lemma}
\label{lem:Solution}
Let  $I = (E, \cC, c,p, \beta)$  be a \textnormal{BC} instance, let  $0<\eps<\frac{1}{2}$,  and 
let $R$ be an \textnormal{SRS} of $I$ and $\eps$. Then $R$ is a representative set of $I$ and $\eps$. 
\end{lemma}


		
	
The proof of Lemma~\ref{lem:Solution} is given in Appendix~\ref{sec:omitted-alg}.
We proceed to construct an  SRS whose cardinality depends only on $\eps$. First, we partition the profitable elements (and possibly some more elements) into a small number of {\em profit classes}, where elements from the same profit class have {\em similar} profits. 
The profit classes are derived from a $2$-approximation $\alpha$ for $\OPT(I)$, which can be easily computed in polynomial time. 
Specifically, for all $r \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]$ define the $r$-{\em profit class} as 
\begin{equation}
	\label{Er}
%	\kappa_{r}(\alpha)
{\ck}_{r}(\alpha)
 = \left\{e \in E~\bigg|~ \frac{ p(e)}{2 \cdot \alpha} \in \big( (1-\eps)^{r}, (1-\eps)^{r-1} \big]\right\}.
\end{equation} %and the independent sets are $\{A \subseteq C_{r}(\alpha)~|~A \in \cI_{\leq q(\eps)}\}$

%For each  
%$r \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]$, we define $\left[ (E, \cI_2) \cap C_{r}(\alpha) \right]_{\leq q(\eps)}$, the {\em corresponding matroid} for the
%$r$-profit class.
%Our construction of the representative set is iterative. In each iteration, we construct a variation of a representative for a single matroid by computing a minimum basis w.r.t. the cost function $c$, for the matroid defined as the union of the corresponding matroids of all profit classes. Note that by Lemma~\ref{lem:prel} the latter is a matroid. This may not be enough to construct a representative set. To do so, for each  
 %and return the union of bases across all profit classes. %all elements $e \in E$ such that  $\frac{p(e)}{2\alpha} \in \big( (1-\eps)^{r}, (1-\eps)^{r-1} \big]$ 
%The pseudocode of algorithm $\textsf{FindRep}$, which outputs a representative set, is given in Algorithm~\ref{alg:representative}.
 
In the following, we give a definition of an {\em exchange set} for each profit class.  This facilitates the construction of an SRS.   
In words, a subset of elements $X$ is an exchange set for some profit class ${\ck}_r(\alpha)$ if any feasible set $\Delta$ and element $a \in (\Delta \cap {\ck}_r(\alpha)) \setminus X$ can be replaced (while maintaining feasibility) by some element $b \in (X \cap {\ck}_r(\alpha)) \setminus \Delta$ such that the cost of $b$ is no larger than the cost of $a$. Formally, 
\begin{definition}
 	\label{def:r-set}
 	Let $I = (E, \cC, c,p, \beta)$ be a \textnormal{BC} instance, $0<\eps<\frac{1}{2}$, $\frac{\OPT(I)}{2} \leq \alpha \leq \OPT(I)$, $r \in [\log_{1-\eps}\left(\frac{\eps}{2}\right)+1]$, and $X \subseteq {\ck}_r(\alpha)$. We say that $X$ is an {\em exchange set} for $I,\eps,\alpha,$ and $r$ if: 
 \begin{itemize}
\item For all $\Delta \in \cm_{\leq q(\eps)}$ and $a \in (\Delta \cap {\ck}_r(\alpha)) \setminus X$ there is $b \in ({\ck}_r(\alpha) \cap X) \setminus \Delta$ satisfying 
\begin{itemize}
\item $c(b) \leq c(a)$.
\item $\Delta-a+b \in \cm_{\leq q(\eps)}$.
\end{itemize} 
\end{itemize}

 
 \end{definition}
 
 The similarity between SRS and exchange sets is not coincidental. We show that if a set $R \subseteq E$ satisfies that $R \cap {\ck}_r(\alpha)$ is an exchange set for any $r \in [\log_{1-\eps}\left(\frac{\eps}{2}\right)+1]$, then $R$ is an SRS, and thus also a representative set by Lemma~\ref{lem:Solution}. This allows us to construct an SRS using a union of disjoint exchange sets, one for each profit class. 
 \begin{lemma}
\label{lem:sufficientRep}
	Let $I = (E, \cC, c,p, \beta)$ be a \textnormal{BC} instance, $0<\eps<\frac{1}{2}$, $\frac{\OPT(I)}{2} \leq \alpha \leq \OPT(I)$ and $R \subseteq E$. If for all $r \in [\log_{1-\eps}\left(\frac{\eps}{2}\right)+1]$ it holds that $R \cap {\ck}_r(\alpha)$ is an  exchange set for $I,\eps,\alpha,$ and $r$, then $R$ is a representative set of $I$ and $\eps$. 
\end{lemma} 

We give the formal proof in Appendix~\ref{sec:omitted-alg}.  
We now present a unified algorithm for finding a representative set for both types of constraints, namely, matching or matroid intersection constraints. This is achieved by taking the union of exchange sets of all profit classes. Nevertheless, for the construction of exchange sets we distinguish between the two types of constraints.
This results also in different sizes for 
the obtained representative sets. Our algorithms for finding the exchange sets are the core technical contribution of this paper. 

For matching constraints, we design an algorithm which constructs an exchange set for any profit class by finding multiple matchings of $\cC$ from the given profit class. Each matching has a bounded cardinality, and the edges are chosen using a greedy approach to minimize the cost. 
We give the full details and a formal proof of Lemma~\ref{lem:mainMatching} in Section~\ref{sec:lemMainProofMatching}. 
\begin{lemma}
	\label{lem:mainMatching}
	There is an algorithm $\textnormal{\textsf{ExSet-Matching}}$ that given a \textnormal{BM} instance $I$, $0<\eps <\frac{1}{2}$, $\frac{\OPT(I)}{2} \leq \alpha \leq \OPT(I)$, and $r \in [\log_{1-\eps}\left(\frac{\eps}{2}\right)+1]$, 
	returns in time $q(\eps) \cdot \textnormal{poly}(|I|)$ an exchange set $X$ for $I,\eps,\alpha,$ and $r$, such that $|X| \leq 18 \cdot {q(\eps)}^2$. 
\end{lemma} 

Our algorithm for matroid intersection constraints is more involved and generates an exchange set by an {\em asymmetric interpretation} of the two given matroids. {\bf This technique was first described by \cite{huang2020fpt} and thus the proof of the next lemma follows from Theorem 3.6 in \cite{huang2020fpt}.} %; we give the following details for completeness.  
 For completeness, we give the full details in Section~\ref{sec:lemMainProof} and a formal proof of Lemma~\ref{lem:mainMatroid} in Appendix~\ref{sec:omitted-matroid}. 
 %Section~\ref{sec:lemMainProof}.
\begin{lemma}
	\label{lem:mainMatroid}
	There is an algorithm $\textnormal{\textsf{ExSet-MatroidIntersection}}$ that given a \textnormal{BI} instance $I$, $0<\eps <\frac{1}{2}$, $\frac{\OPT(I)}{2} \leq \alpha \leq \OPT(I)$, and $r \in [\log_{1-\eps}\left(\frac{\eps}{2}\right)+1]$, 
	returns in time  ${q(\eps)}^{O(q(\eps))} \cdot \textnormal{poly}(|I|)$ an exchange set $X$ for $I,\eps,\alpha,$ and $r$, such that $|X| \leq {q(\eps)}^{O(q(\eps))}$. 
\end{lemma} 






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


 Using the above, we design 
 an algorithm that returns a representative set for both types of constraints. This is done by computing the $2$-approximation $\alpha$ of $\OPT(I)$, and then finding exchange sets for  all profit classes, for the corresponding type of constraint. Finally, we return the union of the above exchange sets. The pseudocode of our algorithm, 
 {\sf RepSet}, is given in Algorithm~\ref{alg:findRep}. 
 
 
 \begin{algorithm}[h]
 	\caption{$\textsf{RepSet}(I = (E, \cC, c,p, \beta),\eps)$}
 	\label{alg:findRep}
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}

\Input{A BC instance $I$ and error parameter $0<\eps<\frac{1}{2}$.}

\Output{A representative set $R$ of $I$ and $\eps$.}

Compute a $2$-approximation $S^*$ for $I$ using a PTAS for BC with parameter $\eps' = \frac{1}{2}$.\label{step:REPAPP}

Set $\alpha \leftarrow p(S^*)$. \label{step:REPalpha}

	Initialize $R \leftarrow \emptyset$.
	
	
	\For{$r \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]$\label{step:REPforr}}{

 \eIf{$I$\textnormal{ is a BM instance}}{$R \leftarrow R \cup \textsf{ExSet-Matching}(I,\eps,\alpha,r)$\label{step:match}.  
 
}{$R \leftarrow R \cup \textsf{ExSet-MatroidIntersection}(I,\eps,\alpha,r)$\label{step:matroid}.


}
}

Return $R$.\label{step:REPret}
 \end{algorithm}
 
 
 
 \begin{lemma}
 	\label{lem:main}
 	  Given a \textnormal{BC} instance $I = (E, \cC, c,p, \beta)$ and $0<\eps <\frac{1}{2}$, Algorithm ~\ref{alg:findRep}  
 	returns a representative set $R$ of $I$ and $\eps$, such that one of the following holds. \begin{itemize}
 		\item If $\cC$ is a matching constraint the running time is $q(\eps)^2 \cdot \textnormal{poly}(|I|)$, and $|R| \leq 54 \cdot q(\eps)^3$. 
 		
 		\item If $\cC$ is a matroid intersection constraint the running time is ${q(\eps)}^{O(q(\eps))} \cdot \textnormal{poly}(|I|)$, and $|R| \leq {q(\eps)}^{O(q(\eps))}$. 
 	\end{itemize} 
 \end{lemma} The proof of the lemma is given in Appendix~\ref{sec:omitted-alg}. 
% \begin{proof}
% 		Let $\alpha$ be the result of Step~\ref{step:REPalpha} of Algorithm~\ref{alg:findRep} and $r \in  [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]$. We distinguish between two cases, depending on the type of constraint. If $I$ is a BM instance then, by Lemma~\ref{lem:mainMatching}, $ \textsf{ExSet-Matching}(I,\eps,\alpha,r)$ is an exchange set for $I,\eps,\alpha$, and $r$ such that $\left|     \textsf{ExSet-Matching}(I,\eps,\alpha,r)    \right| \leq 18 \cdot {q(\eps)}^2$. Therefore, by
% 		Algorithm~\ref{alg:findRep}, it holds that $R \cap {\ck}_r(\alpha)$ is an exchange set for $I,\eps,\alpha$, for all $r \in  [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]$ such that $|R| \leq \left( \log_{1-\eps} \left(\frac{\eps}{2}\right)+1\right)  \cdot 18 \cdot q(\eps)^2$.  Then, by Lemma~\ref{lem:sufficientRep}, $R$ is a representative set of $I$ and $\eps$. 
% 		
% 		For the running time analysis, observe that Step~\ref{step:REPAPP} can be computed in time $\textnormal{poly}(|I|)$ using a PTAS for BC with
% 		an error parameter $\eps= \frac{1}{2}$ (see~\cite{BBGS11}). In addition, each iteration of the \textbf{for} loop of Step~\ref{step:REPforr} can be computed in time $q(\eps) \cdot \textnormal{poly}(|I|)$ by Lemma~\ref{lem:mainMatching}. Hence, as we have $\left(\log_{1-\eps} \left(\frac{\eps}{2}\right)\right)+1$ iterations of the  \textbf{for} loop of Step~\ref{step:REPforr} , the running time of the algorithm is bounded by $ \left( \log_{1-\eps} \left(\frac{\eps}{2}\right)+1\right)  \cdot q(\eps) \cdot  \textnormal{poly}(|I|) \leq 6 \cdot \eps^{-2} \cdot q(\eps) \cdot  \textnormal{poly}(|I|) \leq q(\eps)^2 \cdot \textnormal{poly}(|I|)$. We show more rigorously that $\log_{1-\eps} \left(\frac{\eps}{2}\right) +1 \leq 3 \cdot \eps^{-2}$ in Appendix~\ref{sec:omitted-alg}. It follows that $|R| \leq 3 \cdot \eps^{-2} \cdot 18 \cdot q(\eps)^2 \leq 54 \cdot {q(\eps)}^3$. The proof of the complementary case, where $I$ is a BI instance, is similar. We give the details in Appendix~\ref{sec:omitted-alg}.
% \end{proof}
%
 Next, we use a result of \cite{BBGS11} for adding elements of smaller profits to the solution. The techniques of \cite{BBGS11} are based on a non-trivial patching of two solutions of the Lagrangian relaxation of BC (both for matching and matroid intersection constraints). This approach yields a feasible set with almost optimal profit, where in the worst case the difference from the optimum is twice the 
 maximal profit of an element in the instance. Since we use the latter approach only for non-profitable elements, this effectively does not harm our approximation guarantee. The following is a compact statement of the above result 
 of~ \cite{BBGS11}.
\begin{lemma}
	\label{lem:grandoni}
	 There is a polynomial-time algorithm $\textnormal{\textsf{NonProfitableSolver}}$ that given a \textnormal{BC} instance $I = (E, \cC, c,p, \beta)$ computes a solution $S$ for $I$ of profit $p(S) \geq \OPT(I)-2 \cdot \max_{e \in E} p(e)$.
\end{lemma}



Using the algorithm above and our algorithm for computing a representative set, we obtain an EPTAS for BC. Let $R$ be the representative set returned by $\textsf{RepSet} (I,\eps)$. Our scheme enumerates over subsets of $R$ to select profitable elements for the solution. Using algorithm $\textnormal{\textsf{NonProfitableSolver}}$ of \cite{BBGS11}, the solution is extended to include also non-profitable elements. Specifically, let $\frac{\OPT(I)}{2} \leq \alpha \leq \OPT(I)$ be a $2$-approximation for the optimal profit for $I$. In addition, let $E(\alpha) = \{e \in E~|~ p(e) \leq 2\eps \cdot \alpha\}$ be the set 
including the non-profitable elements, and possibly also profitable elements $e \in E$ 
such that $p(e) \leq 2 \eps \cdot \OPT(I)$. Given a feasible set $F \in \cm$, we define a residual BC instance containing elements which can {\em extend} $F$ by adding elements from $E(\alpha)$. More formally, 

\begin{definition}
	\label{def:instance}
	Given a \textnormal{BC} instance $I = (E, \cC, c,p, \beta)$, $\frac{\OPT(I)}{2} \leq \alpha \leq \OPT(I)$, and $F \in \cm(\cC)$, the {\em residual instance of $F$ and $\alpha$} for $I$ is the \textnormal{BC} instance $I_F(\alpha) = (E_F,\cC_F,c_F,p_F,\beta_F)$ defined as follows. 
	\begin{itemize}
		%\item $V_F = V \setminus V(F)$.
		
		\item $E_F = E(\alpha) \setminus F$.
		
%		\item  $\cI^F_1 = \{A \subseteq E_F ~|~ A \cup F \in \cI_1\}$
		
		%\item If $\cC$ is a matching constraint: $\cC_F = (V(\cC),E'_F)$, where $E'_F = \{\{u,v\} \in E_F~|~u,v \notin V(F)\}$. 
		
		\item $\cC_F = \cC / F$. 
		
	%	\item If $\cC$ is a matroid intersection constraint: $\cC_F = (\cI^F_1 ,\cI^F_2)$, where $\cI^F_1= \{S \subseteq E_F~|~ S \cup F \in \cI_1\}$ and $\cI^F_2= \{S \subseteq E_F~|~ S \cup F \in \cI_2\}$. 
			%\item  $\cm_F = \{A \subseteq E_F ~|~ A \cup F \in \cm\}$. 
		%		\item If $c(F) = B$, then $\forall e \in E_F: p_F(e) = B+1$. Otherwise, $ \forall e \in E_F: p_F(e) = \frac{1}{B-c(F)} \cdot c(e)$. 
		\item $p_F = p|_F$ (i.e., the restriction of $p$ to $F$). 
		
			\item $c_F = c|_F$.
	%	\item $\forall e \in E_F: p_F(e) = p(e)$.
		
	%	\item $\forall e \in E_F: w_F(e) = w(e)$.
		
		\item $\beta_F = \beta-c(F)$. 
	\end{itemize}
	
	
	
	
\end{definition}
\begin{observation}
	\label{ob:residual}
	Let $I = (E, \cC, c,p, \beta)$ be a \textnormal{BC} instance, $\frac{\OPT(I)}{2} \leq \alpha \leq \OPT(I)$, $F \in \cm(\cC)$, and let $T$ be a solution for $I_F(\alpha)$. Then, $T \cup F$ is a solution for $I$. 
\end{observation}

For all solutions $F \subseteq R$ for $I$ with $|F| \leq \eps^{-1}$, we find a solution $T_F$ for the residual instance $I_F(\alpha)$ using Algorithm $\textnormal{\textsf{NonProfitableSolver}}$ and define $K_F =  T_F \cup F$ as the  {\em extended solution} of $F$. 
Our scheme iterates over the extended solutions $K_F$ for all such solutions $F$ and chooses
an extended solution $K_{F^*}$ of maximal total profit. The pseudocode of the scheme is given in Algorithm~\ref{alg:EPTAS}.	

\begin{algorithm}[h]
	\caption{$\textsf{EPTAS}(I = (E, \cC, c,p, \beta),\eps)$}
	\label{alg:EPTAS}
	%Compute the instance $\mathcal{J} = (I,\cG,s,\bar{p},m,c)$. 
	
	%Construct $q,T$ using a $2$-approximation for BMI. 
	
	\SetKwInOut{Input}{input}
	
	\SetKwInOut{Output}{output}
	
	\Input{A BC instance $I$ and an error parameter $0<\eps<\frac{1}{2}$.}
	
	\Output{A solution for $I$.}
	
	Construct the representative set $R \leftarrow \textsf{RepSet} (I,\eps)$.\label{step:rep}
	
	Compute a $2$-approximation $S^*$ for $I$ using a PTAS for BC with parameter $\eps' = \frac{1}{2}$.\label{step:APP2}
	
	Set $\alpha \leftarrow p(S^*)$.
	%Compute a $2$-approximation $S^*$ for $I$ using a PTAS for BMI with $\eps' = \frac{1}{2}$ and set $\alpha = p(S^*)$.\label{step:APP2}
	%Compute a $2$-approximation $S^* = \textsf{PTAS}(\cI,\frac{1}{2})$ for $I$ and set $\alpha = p(S^*)$.\label{step:APP2}
	
	Initialize an empty solution $A \leftarrow \emptyset$.\label{step:init}
	
	\For{$F \subseteq R \textnormal{ s.t. } |F| \leq \eps^{-1} \textnormal{ and } F \textnormal{ is a solution of } I $ \label{step:for}}{
		
		%\in \cI ~\& ~s(F) \leq 1
		
		
		%Find a basic optimal solution $\bar{\lambda}^F$ of $\textnormal{LP}(\cI,F,\alpha)$.\label{step:vertex}
		
		Find a solution for $I_F(\alpha)$ by $T_F \leftarrow \textnormal{\textsf{NonProfitableSolver}}(I_F(\alpha))$.\label{step:vertex}
		
		Let $K_F \leftarrow T_F \cup F$.\label{step:Cf}
		
		
		\If{$p\left(K_F\right) > p(A)$\label{step:iff}}{
			
			Update $A \leftarrow K_F$\label{step:update}
			
		} 
		
		
	}
	
	Return $A$.\label{step:retA}
\end{algorithm}

The running time of Algorithm~\ref{alg:EPTAS} crucially depends on the cardinality of the representative set. Roughly speaking, the running time 
is the number of subsets of the representative set containing at most $\eps^{-1}$ elements, multiplied by a computation time that is polynomial
in the encoding size of the instance. Moreover, since $R = \textsf{RepSet} (I,\eps)$ is a representative set (by Lemma~\ref{lem:main}), there is an almost optimal solution $S$ of $I$ such that the profitable elements in $S$ are a subset of $R$. Thus, there is an iteration of the {\bf for} loop in Algorithm~\ref{alg:EPTAS} such that $F = S \cap H$. In the proof of Lemma~\ref{thm:EPTAS} we focus on this  iteration and show that it yields a solution $K_{F}$ of $I$ with an almost optimal profit. 

\begin{lemma}
	\label{thm:EPTAS}
	Given a \textnormal{BC} instance $I = (E, \cC, c,p, \beta)$ and $0<\eps<\frac{1}{2}$, Algorithm~\ref{alg:EPTAS} returns a solution for $I$ of profit at least $(1-8\eps) \cdot \OPT(I)$ such that one of the following holds. \begin{itemize}
		
			\item  If $I$ is a \textnormal{BM} instance the running time is $2^{ O \left(\eps^{-2} \log \frac{1}{\eps} \right)} \cdot \textnormal{poly}(|I|)$.
		
		\item If $I$ is a \textnormal{BI} instance the running time is ${q(\eps)}^{O(\eps^{-1} \cdot q(\eps))} \cdot \textnormal{poly}(|I|)$, where $q(\eps) = \ceil{\eps^{-\eps^{-1}}}$. 
		
	\end{itemize}
\end{lemma}


The proof of Lemma~\ref{thm:EPTAS} is given in Appendix~\ref{sec:omitted-alg}. We can now prove our main results.

\noindent{\bf Proofs of Theorem~\ref{thm:matching} and Theorem~\ref{thm:matroid}:}  Given a BC instance $I$ and $0<\eps<\frac{1}{2}$, using Algorithm~\ref{alg:EPTAS} for $I$ with parameter $\frac{\eps}{8}$ we have by Lemma~\ref{thm:EPTAS}
the desired approximation guarantee. Furthermore,  
the running time is $2^{ O \left(\eps^{-2} \log \frac{1}{\eps} \right)} \cdot \textnormal{poly}(|I|)$ or ${q(\eps)}^{O(\eps^{-1} \cdot q(\eps))} \cdot \textnormal{poly}(|I|)$, depending on whether $I$ is a BM instance or a BI instance, respectively. 
\qed








==> LP.tex <==
\section{Omitted Proofs}
\label{sec:omitted}

\noindent{\bf Proof of Lemma~\ref{lem:Solution}}: 
As this proof is based on the proof of a corresponding Lemma in \cite{doron2022eptas}, we use some of their definitions and notations. With a slight abuse of notation, 
we use $\OPT$ also to denote the profit of an optimal solution for $I$.
Given an optimal solution, we partition a subset of the elements in the solution 
into $\ceil{\eps^{-1}}$ disjoint sets (some sets may be empty). Specifically,
let $N = \ceil{\eps^{-1}}$; for all $i \in [N]$ define 
\begin{equation}
	\label{J_i}
	J_i = \big\{e \in \OPT~\big|~ p(e) \in \big(\eps^{i} \cdot \OPT(I),  \eps^{i-1} \cdot \OPT(I) \big] \big\}.		
\end{equation} 
Let $i^* = \argmin_{i\in [N]} p(J_i)$. By \eqref{J_i} we have at least 
$\eps^{-1}$ disjoint sets; thus, $p(J_{i^*}) \leq \eps \cdot \OPT(I)$. 
Now, let $L~= ~\bigcup_{k \in  [i^*-1]} J_k$ be the subset of all elements in $\OPT$ 
of profits greater than $\eps^{i^*-1} \cdot \OPT(I)$, and $Q = \OPT \setminus (L \cup J_{i^*})$. 
To complete the proof of the lemma, we need several claims.
\begin{claim}
	\label{clam:Iq}
	$L \in \cm_{\leq q(\eps)}$. 
\end{claim}
%
\begin{claimproof}
	Since $L \subseteq \OPT$, by the hereditary property of $\cm$ we have that $L \in  \cm$. Also, 
	%
	\begin{equation*}
		\label{contradiction1}
		|L| \leq \sum_{e \in L} \frac{p(e)}{\eps^{i^*-1} \cdot \OPT(I)} = \frac{p(L)}{\eps^{i^*-1} \cdot \OPT(I)} \leq  \eps^{- (i^{*}-1)}  \leq   \eps^{-N+1} \leq \eps^{-\eps^{-1}} =  q(\eps)
	\end{equation*} The first inequality holds since $p(e) \geq  \eps^{i^*-1} \cdot \OPT$
	for all $e \in L$. For the second inequality, we note that $L$ is a solution for $I$. By the above it follows that $L \in \cm_{\leq q(\eps)}$. 
\end{claimproof} 
By Claim~\ref{clam:Iq} and as $R$ is a representative set,
it follows that $L$ has a replacement $Z_L \subseteq R$. 
Let $\Delta_L = (L \setminus H) \cup Z_L$. By Property~\ref{p:I} of Definition~\ref{def:Replacement}, we have that $\Delta_L \in \cm_{\leq q(\eps)}$, and it also holds that $\cm_{\leq q(\eps)} \subseteq  \cm$. 
Hence, $\Delta_L \in  \cm$. Furthermore, as $Q \subseteq \OPT$ and  $\OPT \in \cm$, by the 
hereditary property for $\cm$ we have that $Q \in  \cm$. Therefore, by Lemma~\ref{ob:matroid}, there is a subset $T \subseteq Q \setminus\Delta_L$, where $|T|  = \max\{|Q| - 2 \cdot |\Delta_L|,0\}$, such that $\Delta_L \cup T \in \cm$. 

Let $S = \Delta_L \cup T$. We show that $S$ satisfies the conditions of the lemma. 

\begin{claim}
	\label{claim:IsSolution}
	$S$ is a solution for $I$. 
\end{claim}

\begin{claimproof}
	By the definition of $T$ it holds that $S = \Delta_L \cup T \in \cm$. Moreover, 	
	\[
	\begin{array}{ll}
		w(S) &= w(\Delta_L\cup T) \\
		& \leq w(Z_L)+ w(L \setminus H) +w(T) \\
		& \leq w(L \cap H)+w(L \setminus H)+w(T) \\ 
		& \leq w(L)+w(Q) \\ 
		& \leq w(\OPT)\\
		& \leq \beta.
	\end{array}
	\]
	The second inequality holds since $w(Z_L) \leq w(L \cap H)$ (see Property~\ref{p:s} of Definition~\ref{def:Replacement}). For the third inequality, recall that $T \subseteq Q$. The last inequality holds since $\OPT$ is a solution for $I$. 
\end{claimproof} 

The proof of the next claim relies on
the {\em profit gap}  between the elements in $Q$ and $L$. 
\begin{claim}
	\label{clam:profitBound1}
	$p\left(Q \setminus T\right) \leq \eps \cdot \OPT(I)$.
\end{claim}
\begin{claimproof} 
	
	Observe that 
	\begin{equation}
		\label{eq:menS}
		|Q \setminus T| \leq 2 \cdot |\Delta_L| \leq 2 \cdot |Z_L|+2 \cdot |L \setminus H| \leq 2 \cdot |L \cap H|+2 \cdot |L \setminus H| \leq 2 \cdot |L|.
	\end{equation} 
	The first inequality follows from the definition of $T$. For the third inequality, we use Property~\ref{p:car} of Definition~\ref{def:Replacement}. Hence, 
	\begin{equation*}
		\begin{aligned}
			p(Q \setminus T) \leq{} & |Q \setminus T| \cdot \eps^{i^*} \cdot \OPT(I) \leq  2 \cdot |L| \cdot \eps^{i^*} \cdot \OPT(I) \leq 2\eps \cdot p(L) \leq 2\eps \cdot \OPT(I).
		\end{aligned}
	\end{equation*} 
	
	The first inequality holds since $p(e) \leq \eps^{i^*} \cdot \OPT(I)$ for all $e \in Q$. 
	%
	The second inequality is by \eqref{eq:menS}. The third inequality holds since $p(e) > \eps^{i^*-1} \cdot \OPT(I)$ for all $e \in L$. 
\end{claimproof} 	

\begin{claim}
	\label{clam:profitBound2}
	$p\left(S\right) \geq (1-4\eps) \OPT(I)$.
\end{claim} 

\begin{claimproof} 
	%
	By Property~\ref{p:p} of Definition~\ref{def:Replacement},
	\begin{equation}
		\label{eq:proofProfit1}
		\begin{aligned}
			p(\Delta_L) ={} & p((L \setminus H) \cup Z_L) \geq (1-\eps) \cdot p(L).
		\end{aligned}
	\end{equation} Moreover, 
	\begin{equation}
		\label{eq:proofProfit2}
		\begin{aligned}
			p(T) {} & \geq p(Q) - p(Q \setminus T) \geq p(Q) - 2\eps \cdot \OPT(I) \geq (1-\eps) \cdot p(Q) - 2\eps \cdot \OPT(I). 
		\end{aligned}
	\end{equation} 
	
	The second inequality is by Claim~\ref{clam:profitBound1}. Using \eqref{eq:proofProfit1} and \eqref{eq:proofProfit2}, we have that 
	
	\[	
	\begin{array}{ll}
		p(\Delta_L)+p(T) & \geq (1-\eps) \cdot p(L \cup Q)-2\eps \cdot \OPT(I) 
		\\ & = (1-\eps) \cdot p(\OPT \setminus J_{i^*})-2\eps \cdot \OPT(I) \\
		&  \geq (1-\eps) \cdot (1-\eps) \cdot \OPT(I)-2\eps \cdot \OPT(I)\\
		&  \geq (1-4\eps) \cdot \OPT(I). 
	\end{array}
	\]
	
	The second inequality holds since $p(J_{i^*}) \leq \eps \cdot \OPT(I)$. Observe that 
	$S = \Delta_L \cup T$ and $T \cap \Delta_L = \emptyset$. Therefore,  $$p(S) = p(\Delta_L)+p(T) \geq (1-4\eps) \cdot \OPT(I).$$
	
\end{claimproof} 
Finally, we note that, by \eqref{J_i} and the definition of $Q$, it holds that $Q \cap H = \emptyset$. Consequently, by the definition of $S$, we have that $S \cap H \subseteq Z_L$. 
As $Z_L \subseteq R$ (by Definition~\ref{def:Representatives}), it follows that $S \cap H \subseteq R$. Hence, using Claims~\ref{claim:IsSolution} and~\ref{clam:profitBound2},
we have the statement of the lemma.  \qed
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


{\bf Proof of Lemma~\ref{lem:sufficientRep}:}
	For the proof of the lemma, we define a {\em substitution} of some independent set as in \cite{doron2022eptas}. The first two properties of substitution of some $G \in \cm_{\leq q(\eps)}$ are identical to the first two properties in the definition of a replacement of $G$. 
	However, we require that a substitution preserves the number of profitable elements in $G$ from each profit class, and that a substitution must be disjoint to the set of non-profitable elements in $G$. %
	
	\begin{definition}
		\label{def:sub}
		For $G \in \cm_{\leq q(\eps)}$ and $Z_G \subseteq \bigcup_{r \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1] } C_r(\alpha)$, we say that $Z_G$ is a {\em substitution} of $G$ if the following holds. \begin{enumerate}
			
			
			\item $(G \setminus H) \cup Z_G \in \cm_{\leq q(\eps)}$.\label{pp:1}
			
			\item  $w(Z_G) \leq w(G \cap H)$.\label{pp:2}
			
			\item For all $r \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]$ it holds that $|C_r(\alpha) \cap Z_G| = |C_r(\alpha) \cap G \cap H|$.\label{pp:3} 
			
			
			\item $(G \setminus H) \cap Z_G = \emptyset$.\label{pp:4}
			%
		\end{enumerate}
	\end{definition}
	\begin{claim}
		\label{claim:substitution}
		For any $G \in \cm_{\leq q(\eps)}$ there is a substitution $Z_G$ of $G$ such that $Z_G \subseteq R$. 
	\end{claim}
	\begin{claimproof}
		Let $G \in \cm_{\leq q(\eps)}$ and let $Z_G$ be a substitution of $G$ such that $|Z_G \cap R|$ is maximal among all substitutions of $G$; formally, let $\mathcal{S}(G)$ be all substitutions of $G$ and let $Z_G \in \{ Z \in \mathcal{S}(G)~|~ |Z \cap R| = \max_{Z' \in \mathcal{S}(G)} |Z' \cap R|\}$. Since $G \cap H$ is in particular a substitution of $G$  it follows that $\mathcal{S}(G)\neq \emptyset$, and thus  $Z_G$ is well defined.  Assume towards a contradiction that there is $a \in Z_G \setminus R$; then, by Definition~\ref{def:sub} there is $r \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]$ such that $a \in C_r(\alpha)$. Let $\Delta_G = (G \setminus H) \cup Z_G$; by definition~\ref{def:sub} it holds that $\Delta_G \in \cm_{\leq q(\eps)}$. In addition, because $R$ is exchangeable for $I,\eps,\alpha$, and $r$, by Definition~\ref{def:r-set} there is $b \in C_r(\alpha) \cap R \setminus \Delta_G$ such that $w(b) \leq w(a)$ and $\Delta_G -a+b \in \cm_{\leq q(\eps)}$. Then,  the properties of Definition~\ref{def:sub} are satisfied for $Z_G-a+b$ by the following. \begin{enumerate}
			\item $(G\setminus H) \cup (Z_G -a +b) =  \Delta_G-a+b \in \cm_{\leq q(\eps)}$ by the definition of $b$. 
			
			\item  $w(Z_G-a+b) \leq w(Z_G) \leq w(G\cap H)$ because $w(b) \leq w(a)$. 
			
			\item for all $r' \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]$ it holds that $|C_{r'}(\alpha) \cap (Z_G-a+b)| = |C_{r'}(\alpha) \cap Z_G| = |C_{r'}(\alpha) \cap G \cap H|$ because $a,b \in C_r(\alpha)$.
			
			\item $|(G \setminus H) \cap (Z_G -a+b)| \leq |(G \setminus H) \cap (Z_G)| = 0$ where the inequality follows because $b \notin \Delta_G$ and the equality is since $Z_G$ is a substitution of $G$. 
		\end{enumerate}
		
		By the above and Definition~\ref{def:sub}, it follows that $Z_G+a-b$ is a substitution of $G$; that is, $Z_G+a-b \in \mathcal{S}(G)$. Moreover, \begin{equation}
			\label{eq:ZG}
			|R \cap (Z_G -a+b)|>|R \cap Z_G| = \max_{Z \in \mathcal{S}(G)} |Z \cap R|.
		\end{equation} The first inequality is because $a \in Z_G \setminus R$ and $b \in R$. By \eqref{eq:ZG} we reach a contradiction since we found a substitution of $G$ with more elements in $R$ than $Z_G \in \mathcal{S}(G)$, which is defined as a substitution of $G$ with maximal number of elements in $R$. Therefore, $Z_G \subseteq R$ as required.
		\end{claimproof}
	 %$Z_G \in \mathcal{S}(G)$. 
	%


\begin{claim}
	\label{claim:RR}
	For all $e \in H$ there is exactly one $r \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]$ such that $e \in C_r(\alpha)$.
\end{claim}
\begin{claimproof}
	Let $e \in H$. Observe that: \begin{equation}
		\label{eq:app}
		\frac{\eps}{2} \leq \frac{p(e)}{2 \cdot \OPT(I)} \leq \frac{p(e)}{2 \cdot \alpha} \leq \frac{p(e)}{\OPT(I)} \leq 1.
	\end{equation}The first inequality holds since $e \in H$. The second and third inequalities are because $\alpha$ is the value of a $2$-approximation for the optimum of $I$; thus, $\frac{\OPT(I)}{2} \leq \alpha \leq \OPT(I)$. The last inequality is because $\{e\}$ is a solution of $I$ (or this element can be discarded from the instance as it cannot appear in any solution of $I$). In addition, observe that for $r_0 = \ceil{\log_{1-\eps} \frac{\eps}{2}}$ it holds that $(1-\eps)^{r_0} \leq \frac{\eps}{2}$ and that for $r_1 = 1$ it holds that $(1-\eps)^{r_1-1} = 1$. Hence, because $r_0 \leq \floor{\log_{1-\eps} \left(\frac{\eps}{2}\right)+1}$, by \eqref{eq:app}, there is exactly one $r \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]$ such that $\frac{p(e)}{2\alpha} \in \big((1-\eps)^r, (1-\eps)^{r-1}\big]$; thus, by \eqref{Er} it holds that $e \in C_r(\alpha)$ and $e \notin C_{r'}(\alpha)$ for $r' \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1] \setminus \{r\}$.  
\end{claimproof}

We are now ready to prove Lemma~\ref{lem:sufficientRep}. The proof follows by showing that for any $G \in \cm_{\leq q(\eps)}$ a substitution of $G$ which is a subset of $R$ is in fact a replacement of $G$. Let $G \in \cm_{\leq q(\eps)}$; by Claim~\ref{claim:substitution}, $G$ has a substitution $Z_G \subseteq R$. Then, \begin{equation}
	\label{eq:profitR}
	\begin{aligned}
		p(Z_G) \geq{} & \sum_{r \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]} p(C_r(\alpha) \cap Z_G) 
		\\ \geq{} &  \sum_{r \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1] \text{ s.t. } C_r(\alpha) \neq \emptyset} |C_r(\alpha) \cap Z_G| \cdot \min_{e \in C_r(\alpha)} p(e) 
		\\ \geq{} & \sum_{r \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1] \text{ s.t. } C_r(\alpha) \neq \emptyset} |C_r(\alpha) \cap G \cap H| \cdot (1-\eps) \cdot \max_{e \in C_r(\alpha)} p(e) 
		\\ \geq{} & (1-\eps) \cdot p(G \cap H).
	\end{aligned}
\end{equation}  The third inequality is by \eqref{Er} and Property~\ref{pp:3} of Definition~\ref{def:sub}. The last inequality follows from Claim~\ref{claim:RR}. Therefore,  
\begin{equation}
	\label{eq:profitFINAL}
	\begin{aligned}
		p((G \setminus H) \cup Z_G) & = p(G \setminus H)+p(Z_G) \\
		&  \geq p(G \setminus H)+(1-\eps) \cdot p(G \cap H) \\
		& \geq (1-\eps) \cdot p(G).
	\end{aligned}
\end{equation}
The first equality follows by Property~\ref{pp:4} of Definition~\ref{def:sub}. The first inequality is by \eqref{eq:profitR}. Now,  $Z_G$ satisfies Property~\ref{p:I} and~\ref{p:s} of Definition~\ref{def:Replacement} by Properties~\ref{pp:1},~\ref{pp:2} of Definition~\ref{def:sub}, respectively. In addition, $Z_G$ satisfies Property~\ref{p:p} of Definition~\ref{def:Replacement} by \eqref{eq:profitFINAL}. Finally, $Z_G$ satisfies Property~\ref{p:car}  of Definition~\ref{def:Replacement} by $$|Z_G| = \sum_{r \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]} |Z_G \cap C_r(\alpha)| \leq \sum_{r \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]} |G \cap H \cap C_r(\alpha)| = |G \cap H|.$$ The first inequality holds since $Z_G$ is a substitution of $G$. The last equality follows from Claim~\ref{claim:RR}. We conclude that $Z_G$ is a replacement of $G$ such that $Z_G \subseteq R$; thus, $R$ is a representative set by Definition~\ref{def:Representatives}. \qed











	In the following proofs we rely on the next technical auxiliary claim. \begin{claim}
	\label{claim:log}
	For all $0<\eps<\frac{1}{2}$ it holds that $\log_{1-\eps} \left(\frac{\eps}{2}\right)+1 \leq 3 \eps^{-2}$.
\end{claim}
\begin{claimproof}
	Using logarithm rules we have
	% 
	\begin{equation*}
		\label{eq:log1}
		\log_{1-\eps} \left(\frac{\eps}{2}\right)+1  \leq 
		%
		\frac{\ln \left(\frac{2}{\eps}\right)}{-\ln \left(1-\eps \right)}+1 \leq \frac{2\eps^{-1}}{\eps}+1 \leq 3 \eps^{-2}. 
	\end{equation*} 
	The second inequality follows from  $x< -\ln (1-x), \forall x>-1, x \neq 0$, and $\ln (y) < y, \forall y>0$. 
\end{claimproof}





{\bf Proof of Lemma~\ref{lem:main}:}
	Let $\alpha$ be the result of Step~\ref{step:REPalpha} of Algorithm~\ref{alg:findRep} and let $r \in  [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]$. We split the proof into two complementary cases depending on the type of constraint of $I$. \begin{itemize}
		\item $\cC$ is a matching constraint. Then, by Lemma~\ref{lem:mainMatching} it holds that $ \textsf{RepMatching}(\cI,\eps,\alpha,r)$ is an exchangeable set for $I,\eps,\alpha$, and $r$ such that $\left|     \textsf{RepMatching}(\cI,\eps,\alpha,r)    \right| \leq 80 \cdot {q(\eps)}^3$. Therefore, by Step~\ref{step:REPforr}, Step~\ref{step:match}, and Step~\ref{step:REPret} of Algorithm~\ref{alg:findRep} it holds that $R$ is an exchangeable set for $I,\eps,\alpha$, and for all $r \in  [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]$ such that $|R| \leq \left( \log_{1-\eps} \left(\frac{\eps}{2}\right)+1\right)  \cdot 80 \cdot q(\eps)^3$.  Then, by Definition~\ref{def:r-set} and Lemma~\ref{lem:sufficientRep} it holds that $R$ is a representative set of $I$ and $\eps$. Moreover, the running time of the algorithm is $\textnormal{poly}(|I|)$ in this case. Step~\ref{step:REPAPP} can be computed in time $\textnormal{poly}(|I|)$ using a PTAS for BC with
		an error parameter $\eps= \frac{1}{2}$ (see~\cite{BBGS11}). In addition, each iteration of the \textbf{for} loop of Step~\ref{step:REPforr} can be computed in time $\textnormal{poly}(|I|)$ by Lemma~\ref{lem:mainMatching}. Hence, as we have $O\left(\log_{1-\eps} \left(\frac{\eps}{2}\right)\right) $ iterations of the  \textbf{for} loop of Step~\ref{step:REPforr} , the running time of the algorithm is $O\left(\log_{1-\eps} \left(\frac{\eps}{2}\right)\right)  \cdot \textnormal{poly}(|I|)$; then, by Claim~\ref{claim:log} the running time is $O(\eps^{-2}) \cdot  \textnormal{poly}(|I|)$  in case that $\cC$ is a matching constraint.
		
		\item $\cC$ is a matroid intersection constraint. By Lemma~\ref{lem:mainMatroid}, $\textsf{RepMatroidIntersection}(\cI,\eps,\alpha,r)$ is an exchangeable set for $I,\eps,\alpha$, and $r$ such that $\left|     \textsf{RepMatroidIntersection}(\cI,\eps,\alpha,r)    \right| \leq {q(\eps)}^{O(q(\eps))}$. Therefore, by Step~\ref{step:REPforr}, Step~\ref{step:matroid}, and Step~\ref{step:REPret} of Algorithm~\ref{alg:findRep} it holds that $R$ is an exchangeable set for $I,\eps,\alpha$, for all $r \in  [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]$ such that $|R| \leq \left( \log_{1-\eps} \left(\frac{\eps}{2}\right)+1\right)  \cdot  {q(\eps)}^{O(q(\eps))}$.  Then, by Definition~\ref{def:r-set} and Lemma~\ref{lem:sufficientRep} it holds that $R$ is a representative set of $I$ and $\eps$. For the running time of the algorithm, observe that Step~\ref{step:REPAPP} can be computed in time $\textnormal{poly}(|I|)$ using a PTAS for BC with
		an error parameter $\eps= \frac{1}{2}$ (see~\cite{BBGS11}). In addition, each iteration of the \textbf{for} loop of Step~\ref{step:REPforr} can be computed in time ${q(\eps)}^{O(q(\eps))} \cdot \textnormal{poly}(|I|)$ by Lemma~\ref{lem:mainMatroid}. Hence, as we have $O\left(\log_{1-\eps} \left(\frac{\eps}{2}\right)\right) $ iterations of the  \textbf{for} loop of Step~\ref{step:REPforr} , the running time of the algorithm is $O\left(\log_{1-\eps} \left(\frac{\eps}{2}\right)\right)  \cdot {q(\eps)}^{O(q(\eps))} \cdot \textnormal{poly}(|I|)$; then, by Claim~\ref{claim:log} it holds that $O\left(\log_{1-\eps} \left(\frac{\eps}{2}\right)\right) = O(\eps^{-2})$ and it follows that $O\left(\log_{1-\eps} \left(\frac{\eps}{2}\right)\right)  = {q(\eps)}^{O(1)}$; thus, the running time of the algorithm is $ {q(\eps)}^{O(q(\eps))} \cdot \textnormal{poly}(|I|)$ and it also follows that $|R| \leq {q(\eps)}^{O(q(\eps))}$ in case that $\cC$ is a matroid intersection constraint. \qed
	\end{itemize}
	










For the proof of Lemma~\ref{thm:EPTAS}, we use the following auxiliary lemmas.  

\begin{lemma}
	\label{thm:aux1}
	Given a \textnormal{BC} instance $I = (E, \cC, w,p, \beta)$ and $0<\eps<\frac{1}{2}$, Algorithm~\ref{alg:EPTAS} returns a solution for $I$ of profit at least $(1-8\eps) \cdot \OPT(I)$.
\end{lemma}

\begin{proof}

	By Lemma~\ref{lem:Solution},  there is a solution $S$ for $I$ such that $S \cap H \subseteq R$, and $p\left(S\right) \geq (1-4\eps) \OPT(I)$. As for all $e \in S \cap H$ we have $p(e) > \eps \cdot \OPT(I)$, and $S$ is a solution for $I$, it follows that $|S \cap H| \leq \eps^{-1}$.
	% Then, by Step~\ref{step:for} of Algorithm~\ref{alg:EPTAS} 
	We note that there is an iteration of Step~\ref{step:for} in which $F = S \cap H$; thus, in Step~\ref{step:vertex} we construct a solution ${\lambda}^{S \cap H}$ of $I_{S \cap H}$ such that: %We use $X(A) = \{e \in E(\alpha) \setminus A~|~ \bar{\lambda}^{A}_e = 1\}$ for every basic solution $\bar{\lambda}^{A}$ computed in Step~\ref{step:vertex} for $A \subseteq R$.  
	\begin{equation}
		\label{eq:finalProfitA}
		\begin{aligned}
			p\left(\lambda^F\right) \geq \OPT(I_{S \cap H})-2 \cdot \max_{e \in E_{S \cap H}} p(e) \geq p(S \setminus H)- 2 \cdot \max_{e \in E_{S \cap H}} p(e) \geq p(S \setminus H)-4\eps \cdot \OPT(I). 
		\end{aligned}
	\end{equation}
	%The first inequality holds since $S \setminus H$ is in particular a solution of the extension instance $I_F$ by Definition~\ref{def:instance}. 
	The first inequality holds by Lemma~\ref{lem:grandoni}. The second inequality holds since $S \setminus H$ is in particular a solution of the extension instance $I_F$ by Definition~\ref{def:instance}. The third inequality holds since for all $e \in E(S \cap H)$ it holds that $p(e) \leq 2\eps \cdot \alpha \leq 2 \eps \cdot \OPT(I)$. Now, recall $K_{S \cap H}$ defined in Step~\ref{step:Cf} of Algorithm~\ref{alg:EPTAS}. 
	\begin{equation}
		\label{eq:finalProfit}
		\begin{aligned}
			p(K_{S \cap H}) ={} & p(S \cap H)+p\left(\lambda^F\right)  \geq  p(S)- 4\eps \cdot \OPT(I) \geq (1-8\eps) \OPT(I).
		\end{aligned}
	\end{equation}
	
	The first inequality uses~\eqref{eq:finalProfitA}. The last inequality is by Lemma~\ref{lem:Solution}.   \begin{claim}
		\label{claim:Cf}
		$A  = \textnormal{\textsf{EPTAS}}(\cI,\eps)$ is a solution of $I$. 
	\end{claim}
	%
	\begin{claimproof} If $A = \emptyset$ the claim trivially follows since $\emptyset$ is a solution of $I$. Otherwise, by Step~\ref{step:update} of Algorithm~\ref{alg:EPTAS}, there is a solution $F$ of $I$ such that $A = K_F$. Observe that by Definition~\ref{def:instance} it holds that $\lambda^F \in \cm(\cC_F)$ and that $\lambda^F \cup F \in \cm(\CC)$; thus, it holds that $K_F \in \cm(\cC)$. Additionally, 
		
		
		%By Observation~\ref{ob:convexHull}, $X(F)$ is an independent set in the matroid $M_{F}(\alpha)$. 
		%Also, recall that $\cm_{F} (\alpha) = \left((E,\cI) /F \right) \cap E(\alpha) $. Hence, by Definition~\ref{def:matroids}, we have that $X(F) \cup F =K_F \in \cI$. 
		
		
		
		%
		$$w\left(K_{F}\right) = w(F)+w\left(\lambda^F\right) = w(F)+ w_F(\lambda^F) \leq w(F)+\beta_F = w(F)+\beta-w(F) = \beta.$$ 
		The inequality is since $\lambda^F$ is a solution for $I_F$. By the above, we conclude that $A$ is a solution for $I$.  
	\end{claimproof} 
	
	By Claim~\ref{claim:Cf}, Steps~\ref{step:for}, \ref{step:update} and~\ref{step:retA}
	of Algorithm~\ref{alg:EPTAS} and \eqref{eq:finalProfit}, we have that
	%
	$A = \textsf{EPTAS}(I,\eps)$ is a solution for $I$ satisfying $p(A) \geq p(K_{S \cap H}) \geq (1-8\eps) \OPT(I)$. This completes the proof. 	
\end{proof}
























%{\bf Proof of Lemma~\ref{thm:running}:}

\begin{lemma}
	\label{thm:aux2}
	Given a \textnormal{BC} instance $I = (E, \cC, w,p, \beta)$ and $0<\eps<\frac{1}{2}$, the running time of Algorithm~\ref{alg:EPTAS} satisfies one of the following. \begin{itemize}
		\item If $\cC$ is a matroid intersection constraint the running time is ${q(\eps)}^{O(\eps^{-1} \cdot q(\eps))} \cdot \textnormal{poly}(|I|)$. 
		
		\item  If $\cC$ is a matching constraint  the running time is $2^{ O \left(\eps^{-2} \log \frac{1}{\eps} \right)} \cdot \textnormal{poly}(|I|)$.
	\end{itemize}
\end{lemma}
\begin{proof}


	For the following, let $$W = 	\big\{F \subseteq R~\big|~ |F| \leq \eps^{-1}, F \in \cm(\cC), w(F) \leq \beta\big\}$$ be the set of solutions considered in Step~\ref{step:for} of Algorithm~\ref{alg:EPTAS}. We split the proof into two parts, based on the type of constraints of $I$. \begin{enumerate}
		\item $\cC$ is a matroid intersection constraint. By Lemma~\ref{lem:main}, the time complexity of Step~\ref{step:rep} 
		%
		is ${q(\eps)}^{O(q(\eps))}  \cdot \textnormal{poly}(|I|)$. In addition, Step~\ref{step:APP2} can be computed in time $\textnormal{poly}(|I|)$, by using a PTAS for BC taking 
		%with parameter 
		$\eps=\frac{1}{2}$ (see~\cite{GZ10}). 
	% Now, Let $$W = 	\big\{F \subseteq R~\big|~ |F| \leq \eps^{-1}, F \in \cm(\cC), c(F) \leq \beta\big\}$$ be the set of solutions considered in Step~\ref{step:for} of Algorithm~\ref{alg:EPTAS}. 
	Then,
		\begin{equation}
			\label{eq:subR11111}
			\begin{aligned}
				|W| \leq{} &  \left(|R|+1\right)^{\eps^{-1}}
				\leq  {\left({q(\eps)}^{O(q(\eps))}\right)}^{\eps^{-1}} = {q(\eps)}^{O(\eps^{-1} \cdot q(\eps))}.
			\end{aligned}
		\end{equation} The second inequality is by Lemma~\ref{lem:main}. Hence, by \eqref{eq:subR11111}, the number of iterations of the {\bf for} loop  in Step~\ref{step:for} is bounded by ${q(\eps)}^{O(\eps^{-1} \cdot q(\eps))}$. In addition, by Lemma~\ref{lem:grandoni}, the running time of each iteration is  $\textnormal{poly}(|I|)$. By the above, the running time of Algorithm~\ref{alg:EPTAS} is ${q(\eps)}^{O(\eps^{-1} \cdot q(\eps))} \cdot \textnormal{poly}(|I|)$  If $\cC$ is a matroid intersection constraint.  
		
		
		
		\item 	$\cC$ is a matching constraint. By Lemma~\ref{lem:main}, the time complexity of Step~\ref{step:rep} 
		%
		is $\textnormal{poly}(|I|)$. Step~\ref{step:APP2} can be computed in time $\textnormal{poly}(|I|)$, by using a PTAS for BC taking 
		%with parameter 
		$\eps=\frac{1}{2}$ (see~\cite{GZ10}). Therefore, \begin{equation}
			\label{eq:R}
			|R| \leq \left(\log_{1-\eps} \left(\frac{\eps}{2}\right)+1\right)  \cdot 80 \cdot q(\eps)^3 \leq 3\eps^{-2} \cdot 80 \eps^{-3\eps^{-1}} \leq 240 \cdot \eps^{-4\eps^{-1}}. 
		\end{equation}
		The first inequality is by Lemma~\ref{lem:main} and that the number of  iterations of the {\bf for} loop  in Step~\ref{step:for} is bounded by $ \left(\log_{1-\eps} \left(\frac{\eps}{2}\right)+1\right)$. The second inequality is by Claim~\ref{claim:log}. Then,
		\begin{equation}
			\label{eq:subR}
			\begin{aligned}
				|W| \leq{} &  \left(|R|+1\right)^{\eps^{-1}}
				\leq  {\left(240 \cdot \eps^{-4\eps^{-1}}+1\right)}^{\eps^{-1}}
				\leq {\left(\eps^{-20\eps^{-2}}\right)} = 2^{ O \left(\eps^{-2} \log \frac{1}{\eps} \right)}.
			\end{aligned}
		\end{equation} The second inequality is by \eqref{eq:R}. Hence, by \eqref{eq:subR}, the number of iterations of the {\bf for} loop  in Step~\ref{step:for} is bounded by $2^{ O \left(\eps^{-2} \log \frac{1}{\eps} \right)}$. In addition, by Lemma~\ref{lem:grandoni}, the running time of each iteration is  $\textnormal{poly}(|I|)$. By the above, the running time of Algorithm~\ref{alg:EPTAS} is $2^{ O \left(\eps^{-2} \log \frac{1}{\eps} \right)} \cdot \textnormal{poly}(|I|)$  If $\cC$ is a matching constraint.  
	\end{enumerate} \end{proof}


{\bf Proof of Lemma~\ref{thm:EPTAS}:} The proof follows by Lemma~\ref{thm:aux1} and Lemma~\ref{thm:aux2}. \qed







==> findRep.tex <==
\section{Properties of \textsf{FindRep}}
\label{sec:findRep}
